A quasi-quadratic vertex Kernel for Cograph edge editing

We provide a $O(k^2 \mathrm{log} k)$ vertex kernel for cograph edge editing. This improves a cubic kernel found by Guillemot, Havet, Paul and Perez [1] which involved four reduction rules. We generalize one of their rules, based on packing of induced paths of length four, by introducing t-modules, which are modules up to t edge modifications. The key fact is that large t-modules cannot be edited more than t times, and this allows to obtain a near quadratic kernel. The extra $\mathrm{log} k$ factor seems tricky to remove as it is necessary in the combinatorial lemma on trees which is central in our proof. Nevertheless, we think that a quadratic bound should be reachable.

==> commandes_perso.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Commandes perso %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\etc}{etc.}

% Guillemets
\newcommand{\ofg}[1]{``#1''}
\RequirePackage{ifthen}

% Centrer

\newlength{\leftsize}
\newlength{\rightsize}
\newcommand{\leftcentersright}[3]{
	\vskip0.1cm
	\settowidth{\leftsize}{#1}%
	\settowidth{\rightsize}{#3}%
	% On place #2 et on recule de sa longueur
	\par\noindent #1\hskip-\leftsize%
	% On centre #3
	\hfill{#2}\hfill
	% On va au bout de la ligne, on recule de la longueur de #4 et
	% on place #4
	\mbox{}\hskip-\rightsize #3\par%
}
\newcommand{\centers}[1]{\leftcentersright{}{#1}{}}
\newcommand{\leftcenters}[2]{\leftcentersright{#1}{#2}{}}

% Parenthèses
\newcommand{\pa}[2][9]{%
	\ifthenelse{#1 = 0}{#2}{}%
	\ifthenelse{#1 = 1}{(#2)}{}%
	\ifthenelse{#1 = 2}{\big(#2\big)}{}%
	\ifthenelse{#1 = 3}{\Big(#2\Big)}{}%
	\ifthenelse{#1 = 4}{\bigg(#2\bigg)}{}%
	\ifthenelse{#1 = 5}{\Bigg(#2\Bigg)}{}%
	\ifthenelse{#1 = 9}{\left(#2\right)}{}%
}

% Des parenthèses autour d'une fraction (très très pratique !).
% Exemple: $ \paf{1}{2} $
\newcommand{\paf}[2]{\left(\f{#1}{#2}\right)}

% Et l'analogue de \tf pour les parenthèses autour d'une fraction:
\newcommand{\patf}[2]{\left({#1}/{#2}\right)}

% On peut aussi vouloir des crochets de la bonne taille plutôt que des 
% parenthèses (analogue de \pa: mêmes recommandations).
% Exemple: $\crochets{ \f{1}{2} x \ln x }$
\newcommand{\crochets}[2][9]{%
	\ifthenelse{#1 = 0}{#2}{}%
	\ifthenelse{#1 = 1}{[#2]}{}%
	\ifthenelse{#1 = 2}{\big[#2\big]}{}%
	\ifthenelse{#1 = 3}{\Big[#2\Big]}{}%
	\ifthenelse{#1 = 4}{\bigg[#2\bigg]}{}%
	\ifthenelse{#1 = 5}{\Bigg[#2\Bigg]}{}%
	\ifthenelse{#1 = 9}{\left[#2\right]}{}%
}
\newcommand{\pac}[2][9]{\crochets[#1]{#2}}		% Synonyme

% Ou pourquoi pas des accolades (analogue de \pa: mêmes recommandations).
\newcommand{\accolades}[2][9]{%
	\ifthenelse{#1 = 0}{#2}{}%
	\ifthenelse{#1 = 1}{\{#2\}}{}%
	\ifthenelse{#1 = 2}{\big\{#2\big\}}{}%
	\ifthenelse{#1 = 3}{\Big\{#2\Big\}}{}%
	\ifthenelse{#1 = 4}{\bigg\{#2\bigg\}}{}%
	\ifthenelse{#1 = 5}{\Bigg\{#2\Bigg\}}{}%
	\ifthenelse{#1 = 9}{\left\{#2\right\}}{}%
}
\newcommand{\paa}[2][9]{\accolades[#1]{#2}}		% Synonyme

% Ou encore des barres pour les valeurs absolues (analogue de \pa: mêmes
% recommandations).
\newcommand{\abs}[2][9]{%
	\ifthenelse{#1 = 0}{#2}{}%
	\ifthenelse{#1 = 1}{|#2|}{}%
	\ifthenelse{#1 = 2}{\big|#2\big|}{}%
	\ifthenelse{#1 = 3}{\Big|#2\Big|}{}%
	\ifthenelse{#1 = 4}{\bigg|#2\bigg|}{}%
	\ifthenelse{#1 = 5}{\Bigg|#2\Bigg|}{}%
	\ifthenelse{#1 = 9}{\left|#2\right|}{}%
}

% La partie entière peut être écrite à l'américaine plutôt qu'avec 
% l'énigmatique fonction 'E'. C'est efficace...
\newcommand{\partieentiere}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\partieentieresup}[1]{\left\lceil#1\right\rceil}

%Nouvelle fraction, plus jolie
\newcommand{\f}[2]{	
	\mathchoice%
		{\dfrac{#1}{#2}}
    	{\dfrac{#1}{#2}}
		{\frac{#1}{#2}}
		{\frac{#1}{#2}}
}
%Passer simplement une fraction en fraction inline
\newcommand{\tf}[2]{{#1}/{#2}}

%%Opérateurs
\newcommand{\grando}[2]{\underset{#1}{\text{O}}\left({#2}\right)} %GrandO
\newcommand{\grandot}[2]{\text{O}_{#1}\left({#2}\right)} %GrandO en mode text
\newcommand{\petito}[2]{\underset{#1}{\text{o}}({#2})} %PetitO
\newcommand{\petitot}[2]{\text{o}_{#1}({#2})} %PetitO en mode text
\DeclareMathOperator{\Argmax}{argmax} %operateur argmax
\newcommand{\argmax}[1]{\ensuremath{\underset{#1}{\Argmax}}}
\newcommand{\argmaxt}[1]{\ensuremath{\Argmax_{#1}}}
\DeclareMathOperator{\Argmin}{argmin} %operateur argmin
\newcommand{\argmin}[1]{\ensuremath{\underset{#1}{\Argmin}}}
\newcommand{\argmint}[1]{\ensuremath{\Argmin_{#1}}}
\DeclareMathOperator{\rk}{rk} %operateur rk
\DeclareMathOperator{\Aut}{Aut} %ensemble des automorphismes.
\DeclareMathOperator{\End}{End} %ensemble des endomorphismes.
\DeclareMathOperator{\Int}{Int} %ensemble des automorphismes intérieurs.
\DeclareMathOperator{\id}{id} %la putain de fonction identité
\newcommand{\cast}[2]{\overline{#1}^{\, #2}}
\newcommand{\uncast}[2]{\underline{#1}_{\, #2}}

\DeclareMathOperator{\diag}{diag} %operateur diag

\DeclareMathOperator{\supp}{supp} % operateur support

%\DeclareMathOperator{\mod}{mod} % operateur modulo
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}


\newcommand{\Min}[1]{\underset{#1}{\min}}
\newcommand{\Max}[1]{\underset{#1}{\max}}
\newcommand{\Inf}[1]{\underset{#1}{\inf}}
\newcommand{\Sup}[1]{\underset{#1}{\sup}}

\newcommand{\ind}{\ensuremath{\mathds{1}}} %indicatrice

\newcommand{\Sum}[2]{\underset{#1}{\overset{#2}{\sum}}} %somme
\newcommand{\Prod}[2]{\underset{#1}{\overset{#2}{\prod}}} %produit
\newcommand{\Tensor}[2]{\underset{#1}{\overset{#2}{\bigotimes}}} %produit de Kronecker

\newcommand{\transpose}[1]{{}^{\mathrm{t}}#1}

% Plus et moins l'infini.
%
% Lorsque l'on écrit $+\infty$, le plus est trop gros. On fait la même 
% remarque avec $-\infty$. Pour contourner ce problème, vous pouvez utiliser
% des macros spécifiques à ces cas-là.
%
% Exemple: $ \sqrt{n} \tvn \pinf $
%
% Attention, n'utilisez jamais \plus et \moins dans vos corrigés.
% Ces macros n'existent que pour définir \pinf et \minf et quelques autres
% bidouilles comme \Rplus.
% Ne les utilisez pas à la place de + et - dans les opérations courantes !

\newcommand{\plus}{\mbox{\protect\raisebox{.2mm}{\tiny{\ensuremath{+}}}}}
\newcommand{\moins}{\mbox{\protect\raisebox{.2mm}{\tiny{\ensuremath{-}}}}}
\newcommand{\pinf}{{\plus\ensuremath{\infty}}}
\newcommand{\minf}{{\moins\ensuremath{\infty}}}

% L'exponentielle et les complexes

\newcommand{\ir}{\mathrm{i}\xspace}	% « i romain »
\newcommand{\jr}{\mathrm{j}\xspace}	% « j romain »
\newcommand{\irmath}{\text{\i}\xspace} % « i romain sans point »
\newcommand{\jrmath}{\text{\j}\xspace} % « j romain sans point »
\newcommand{\ex}[1]{\mathrm{e}^{\,#1}\xspace}

%%Ensembles et combinatoires

%Ensemble avec propriété à droite \{x | blabla\}
\newcommand{\enstq}[2]{\left\{ \left.#1\ \vphantom{#2}\right|\ #2  \right\}}
%meme chose mais avec des crochets
\newcommand{\crotq}[2]{\left[ \left.#1\ \vphantom{#2}\right|\ #2  \right]}
%même chose mais avec des brackets
\newcommand{\bratq}[2]{\left\langle \left.#1\ \vphantom{#2}\right|\ #2  
\right\rangle}
%Intervalles
\newcommand{\TestGauche}[1]{\ifthenelse{\equal{#1}{}}{\minf}{#1}}
\newcommand{\TestDroite}[1]{\ifthenelse{\equal{#1}{}}{\pinf}{#1}}
\newcommand{\intff}[2]{\intxy{#1}{#2}{[}{]}}
\newcommand{\intof}[2]{\intxy{#1}{#2}{]}{]}}
\newcommand{\intfo}[2]{\intxy{#1}{#2}{[}{[}}
\newcommand{\intoo}[2]{\intxy{#1}{#2}{]}{[}}
\newcommand{\intxy}[4]{\ensuremath{\mathchoice
    {\left#3\,\protect\TestGauche{#1}\,;  \protect\TestDroite{#2}\,\right#4}
    {\left#3\,\protect\TestGauche{#1}\,;  \protect\TestDroite{#2}\,\right#4}
    {\left#3\,\protect\TestGauche{#1}\,;\,\protect\TestDroite{#2}\,\right#4}
    {\left#3\,\protect\TestGauche{#1}\,;\,\protect\TestDroite{#2}\,\right#4}
}}  

\newcommand{\intn}[2]{\ensuremath{
		\left\llbracket\, #1\ ;\ #2\,\right\rrbracket
}}
\newcommand{\intnoo}[2]{\ensuremath{
		\left\rrbracket\, #1\ ;\ #2\,\right\llbracket
	}}
\newcommand{\intnof}[2]{\ensuremath{
		\left\rrbracket\, #1\ ;\ #2\,\right\rrbracket
	}}
\newcommand{\intnfo}[2]{\ensuremath{
		\left\llbracket\, #1\ ;\ #2\,\right\llbracket
	}}

\newsavebox{\boite}
\def\debutcom{\begin{lrbox}{\boite}}
\def\fincomg{\end{lrbox}\makebox[0cm][l]{\usebox{\boite}}%
             \hskip\linewidth\hskip-\textwidth}
\def\fincomd{\end{lrbox}\makebox[0cm][r]{\usebox{\boite}}}
\newenvironment{calculs:rcl}[4][2]{%
  	\par\vskip0.1cm\noindent
  	\begin{tabular*}{\linewidth}[t]%
  		{@{}>{\debutcom}l<{\fincomg}@{\extracolsep{\fill}}
		>{$}#2<{$}@{\extracolsep{0pt}}%
		>{$\ }#3<{\ $}%
      		@{\extracolsep{0pt}}>{$}#4<{$}%
      		@{\extracolsep{\fill}}>{\debutcom}r<{\fincomd}@{}}%
	}{%
  	\end{tabular*}\par%
}

\newenvironment{calculs}[1][2]%
        {\begin{calculs:rcl}[#1]{r}{c}{l}}%
        {\end{calculs:rcl}}


\newcommand{\Union}[2]{\underset{#1}{\overset{#2}{\bigcup}}} %Union
\newcommand{\Uniond}[2]{\underset{#1}{\overset{#2}{\biguplus}}} %Union disjointe
\newcommand{\Inter}[2]{\underset{#1}{\overset{#2}{\bigcap}}} %Intersection

%même chose pour les formules logiques
\newcommand{\Conj}[2]{\underset{#1}{\overset{#2}{\bigwedge}}}
\newcommand{\Disj}[2]{\underset{#1}{\overset{#2}{\bigvee}}}


\newcommand{\fct}[5]{\ensuremath{#1 : \left\{\begin{array}{c c c}
#2 & \rightarrow & #3\\
#4 & \mapsto & #5
\end{array}\right.}}


\newcommand{\inner}[1]{\left\langle#1\right\rangle} %produit scalaire pour tout
%avec choix de ce qu'il y a dedans


\DeclareMathOperator{\Vect}{Vect}
%pour les morphismes et fonctions
\DeclareMathOperator{\Kernel}{Ker} %noyau
\DeclareMathOperator{\Image}{Im} %image
\DeclareMathOperator{\dom}{dom}
\if@anglais
	\DeclareMathOperator{\rg}{rk}
\else
	\DeclareMathOperator{\rg}{rg}
\fi

\DeclareMathOperator{\Sp}{Sp} %spectre

% Quelques raccourcis pour manipuler les nombres complexes.
\newcommand{\barre}[1]{\ensuremath{\overline{#1}}}		% Conjugué
\newcommand{\Arg}{\mathop{\rm Arg\,}\nolimits}	% Argument
\renewcommand{\Re}{\mathop{\text{Re}\,}\nolimits}
\renewcommand{\Im}{\mathop{\text{Im}\,}\nolimits}

%ecriture bb
\newcommand{\Abb}{\ensuremath{\mathbb{A}}}
\renewcommand{\Bbb}{\ensuremath{\mathbb{B}}} %\Bbb voulait déjà dire ça mais 
%est obsolète
\newcommand{\Cbb}{\ensuremath{\mathbb{C}}}
\newcommand{\Dbb}{\ensuremath{\mathbb{D}}}
\newcommand{\Ebb}{\ensuremath{\mathbb{E}}}
\newcommand{\Fbb}{\ensuremath{\mathbb{F}}}
\newcommand{\Gbb}{\ensuremath{\mathbb{G}}}
\newcommand{\Hbb}{\ensuremath{\mathbb{H}}}
\newcommand{\Ibb}{\ensuremath{\mathbb{I}}}
\newcommand{\Jbb}{\ensuremath{\mathbb{J}}}
\newcommand{\Kbb}{\ensuremath{\mathbb{K}}}
\newcommand{\Lbb}{\ensuremath{\mathbb{L}}}
\newcommand{\Mbb}{\ensuremath{\mathbb{M}}}
\newcommand{\Nbb}{\ensuremath{\mathbb{N}}}
\newcommand{\Obb}{\ensuremath{\mathbb{O}}}
\newcommand{\Pbb}{\ensuremath{\mathbb{P}}}
\newcommand{\Qbb}{\ensuremath{\mathbb{Q}}}
\newcommand{\Rbb}{\ensuremath{\mathbb{R}}}
\newcommand{\Sbb}{\ensuremath{\mathbb{S}}}
\newcommand{\Tbb}{\ensuremath{\mathbb{T}}}
\newcommand{\Ubb}{\ensuremath{\mathbb{U}}}
\newcommand{\Vbb}{\ensuremath{\mathbb{V}}}
\newcommand{\Wbb}{\ensuremath{\mathbb{W}}}
\newcommand{\Xbb}{\ensuremath{\mathbb{X}}}
\newcommand{\Ybb}{\ensuremath{\mathbb{Y}}}
\newcommand{\Zbb}{\ensuremath{\mathbb{Z}}}


%les caligraphiées
\newcommand{\Acal}{\ensuremath{\mathcal{A}}}
\newcommand{\Bcal}{\ensuremath{\mathcal{B}}}
\newcommand{\Ccal}{\ensuremath{\mathcal{C}}}
\newcommand{\Dcal}{\ensuremath{\mathcal{D}}}
\newcommand{\Ecal}{\ensuremath{\mathcal{E}}}
\newcommand{\Fcal}{\ensuremath{\mathcal{F}}}
\newcommand{\Gcal}{\ensuremath{\mathcal{G}}}
\newcommand{\Hcal}{\ensuremath{\mathcal{H}}}
\newcommand{\Ical}{\ensuremath{\mathcal{I}}}
\newcommand{\Jcal}{\ensuremath{\mathcal{J}}}
\newcommand{\Kcal}{\ensuremath{\mathcal{K}}}
\newcommand{\Lcal}{\ensuremath{\mathcal{L}}}
\newcommand{\Mcal}{\ensuremath{\mathcal{M}}}
\newcommand{\Ncal}{\ensuremath{\mathcal{N}}}
\newcommand{\Ocal}{\ensuremath{\mathcal{O}}}
\newcommand{\Pcal}{\ensuremath{\mathcal{P}}}
\newcommand{\Qcal}{\ensuremath{\mathcal{Q}}}
\newcommand{\Rcal}{\ensuremath{\mathcal{R}}}
\newcommand{\Scal}{\ensuremath{\mathcal{S}}} 
\newcommand{\Tcal}{\ensuremath{\mathcal{T}}}
\newcommand{\Ucal}{\ensuremath{\mathcal{U}}}
\newcommand{\Vcal}{\ensuremath{\mathcal{V}}}
\newcommand{\Wcal}{\ensuremath{\mathcal{W}}}
\newcommand{\Xcal}{\ensuremath{\mathcal{X}}}
\newcommand{\Ycal}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zcal}{\ensuremath{\mathcal{Z}}}

%les caractères ronds
\newcommand{\Ascr}{\ensuremath{\mathscr{A}}}
\newcommand{\Bscr}{\ensuremath{\mathscr{B}}}
\newcommand{\Cscr}{\ensuremath{\mathscr{C}}}
\newcommand{\Dscr}{\ensuremath{\mathscr{D}}}
\newcommand{\Escr}{\ensuremath{\mathscr{E}}}
\newcommand{\Fscr}{\ensuremath{\mathscr{F}}}
\newcommand{\Gscr}{\ensuremath{\mathscr{G}}}
\newcommand{\Hscr}{\ensuremath{\mathscr{H}}}
\newcommand{\Iscr}{\ensuremath{\mathscr{I}}}
\newcommand{\Jscr}{\ensuremath{\mathscr{J}}}
\newcommand{\Kscr}{\ensuremath{\mathscr{K}}}
\newcommand{\Lscr}{\ensuremath{\mathscr{L}}}
\newcommand{\Mscr}{\ensuremath{\mathscr{M}}}
\newcommand{\Nscr}{\ensuremath{\mathscr{N}}}
\newcommand{\Oscr}{\ensuremath{\mathscr{O}}}
\newcommand{\Pscr}{\ensuremath{\mathscr{P}}}
\newcommand{\Qscr}{\ensuremath{\mathscr{Q}}}
\newcommand{\Rscr}{\ensuremath{\mathscr{R}}}
\newcommand{\Sscr}{\ensuremath{\mathscr{S}}} 
\newcommand{\Tscr}{\ensuremath{\mathscr{T}}}
\newcommand{\Uscr}{\ensuremath{\mathscr{U}}}
\newcommand{\Vscr}{\ensuremath{\mathscr{V}}}
\newcommand{\Wscr}{\ensuremath{\mathscr{W}}}
\newcommand{\Xscr}{\ensuremath{\mathscr{X}}}
\newcommand{\Yscr}{\ensuremath{\mathscr{Y}}}
\newcommand{\Zscr}{\ensuremath{\mathscr{Z}}}


%% Les section théoreme
\theoremstyle{definition}
\newtheorem{Thm}{Theorem}[section]
\newtheorem*{Thm*}{Theorem}
\newtheorem{Prop}[Thm]{Proposition}
\newtheorem{Properties}[Thm]{Properties}
\newtheorem{Lem}[Thm]{Lemma}
\newtheorem*{Lem*}{Lemma}
\newtheorem{Cor}[Thm]{Corollary}
\newtheorem{Fait}[Thm]{Fact}
\newtheorem{Claim}[Thm]{Claim}
\newtheorem{App}[Thm]{Application}
\newtheorem{Con}[Thm]{Conjecture}
%\newtheorem{Exo}{Exercise}

\newtheorem{Def}[Thm]{Definition}
\newtheorem*{Def*}{Definition}
\newtheorem{Ex}[Thm]{Example}
\newtheorem*{Ex*}{Example}
\newtheorem*{Sol}{Solution}
\newtheorem*{Notation}{Notation}

\theoremstyle{remark}
\newtheorem{Rk}[Thm]{Remark}
\newtheorem*{Rk*}{Remark}
\newtheorem{Att}[Thm]{Warning}
\newtheorem*{Att*}{Warning}

